MoFM: A Large-Scale Human Motion Foundation Model

Foundation Models (FM) have increasingly drawn the attention of researchers due to their scalability and generalization across diverse tasks. Inspired by the success of FMs and the principles that have driven advancements in Large Language Models (LLMs), we introduce MoFM as a novel Motion Foundation Model. MoFM is designed for the semantic understanding of complex human motions in both time and space. To facilitate large-scale training, MotionBook, a comprehensive human motion dictionary of discretized motions is designed and employed. MotionBook utilizes Thermal Cubes to capture spatio-temporal motion heatmaps, applying principles from discrete variational models to encode human movements into discrete units for a more efficient and scalable representation. MoFM, trained on a large corpus of motion data, provides a foundational backbone adaptable to diverse downstream tasks, supporting paradigms such as one-shot, unsupervised, and supervised tasks. This versatility makes MoFM well-suited for a wide range of motion-based applications.

==> tab/dvae_arch.tex <==
% Table generated by Excel2LaTe\xmarkfrom sheet 'Sheet1'
\iffalse
\begin{table}[h]
  \centering
  \caption{\red{Add caption}}
  \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{lcc}
    \toprule
    \toprule
    \multicolumn{1}{c}{\textbf{Hyper Parameter}} & \textbf{Encoder} & \textbf{Decoder} \\
    \midrule
    Conv(Transpose) Block & 2     & 2 \\
    ResBlock & 2     & 2 \\
    Hiden Size & \xmark    & y \\
    \midrule
    Vocabulary Size & \multicolumn{2}{c}{8192} \\
    Pose Book dimension & \multicolumn{2}{c}{1} \\
    \midrule
    Training epoch & \multicolumn{2}{c}{2} \\
    Batch size & \multicolumn{2}{c}{3} \\
    Weight Decay & \multicolumn{2}{c}{4} \\
    LR Schedular & \multicolumn{2}{c}{5} \\
    Max LR rate & \multicolumn{2}{c}{6} \\
    Min LR rate & \multicolumn{2}{c}{7} \\
    Tempreture rate & \multicolumn{2}{c}{8} \\
    Tempreture Schedular & \multicolumn{2}{c}{9} \\
    Droupout & \multicolumn{2}{c}{0} \\
    Optimizer & \multicolumn{2}{c}{10} \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
  \label{tab:dv_hyper}%
\end{table}%
\fi

% Table generated by Excel2LaTeX from sheet 'dVAE'
\begin{table*}[htbp]
  \centering
  \caption{Model architecture of custom \dV}
  \resizebox{0.75\textwidth}{!}{%
        \begin{tabular}{l|cccccc}
    \toprule
    \toprule
    \multicolumn{1}{p{4.785em}|}{\textbf{Hyper \newline{}Parameter}} & \multicolumn{1}{p{5.645em}}{\centering{\textbf{3D\newline{} Conv. Block}}} & \multicolumn{1}{p{4.215em}}{\centering{\textbf{3D\newline{} ResBlock}}} & \multicolumn{1}{p{5.43em}}{\centering{\textbf{\centering{2D \newline{}Conv. Block}}}} & \multicolumn{1}{p{4.215em}}{\centering{\centering{\textbf{2D\newline{}ResBlock}}}} & \multicolumn{1}{p{5.07em}}{\centering{\textbf{Hidden\newline{} Dimension}}} & \multicolumn{1}{p{5.07em}}{\centering{\textbf{Vocabulary Size}}} \\
    \midrule
    \multicolumn{1}{p{4.785em}|}{\textbf{Encoder}} & 2     & 2     & \xmark & \xmark    & 256   & \xmark\\
    \multicolumn{1}{p{4.785em}|}{\textbf{Pose Book}} & \xmark    & \xmark & \xmark & \xmark & 256   & 8192 \\
    \textbf{Decoder} & \xmark   & \xmark    & 2     & 2     & \xmark    & \xmark\\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
  \label{tab:dv_arch}%
\end{table*}%


==> tab/dve_hyper.tex <==
% Table generated by Excel2LaTeX from sheet 'dVAE'
\begin{table*}[h]
  \centering
  \caption{Hyperparametrs for training of \dV}
  \resizebox{0.75\textwidth}{!}{%
    \begin{tabular}{l|cc|ccccc}
    \toprule
    \toprule
    \multicolumn{1}{p{4.785em}|}{\textbf{Hyper \newline{}Parameter}} & \multicolumn{1}{p{4.215em}}{\centering{\textbf{Training \newline{}Epoch}}} & \textbf{Batch size} & \textbf{Optimizer} & \multicolumn{1}{p{4.645em}}{\centering{\textbf{LR \newline{}Schedular}}} & \multicolumn{1}{p{4.215em}}{\centering{\textbf{Max \newline{}LR rate}}} & \multicolumn{1}{p{4.215em}}{\centering{\textbf{Min\newline{} LR rate}}} & \multicolumn{1}{p{4.215em}}{\centering{\textbf{Warm-up\newline{} Epoch}}} \\
    \midrule
    \textbf{Values} & 20     & 24     & AdamW    & WarmupCosineLR     & 3.0e-4     & 1.0e-6     & 1 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
  \label{tab:dv_hyper}%
\end{table*}%

==> tab/model_size.tex <==
\begin{table}[htbp]
  \centering
  \caption{Model size comparison of ViT and \memt}
  \label{tab:model_size}

\resizebox{\linewidth}{!}{%
    \begin{tabular}{lcc}
    \toprule
    \toprule
    \multicolumn{1}{p{4.57em}}{\centering{\textbf{Model \newline{}Name}}}  & \multicolumn{1}{p{5em}}{\centering{\textbf{Model Size\newline{} (MB)}}} & \multicolumn{1}{p{14.215em}}{\centering{\textbf{Size Increase \newline{}from ViT-Base (\%)}}} \\
    \midrule
    ViT-Base & 86    & - \\
    \memt(Our) & 88    & 2.4 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
}
\end{table}



==> tab/trans_arch.tex <==
% Table generated by Excel2LaTeX from sheet 'Trans_Pre'

\begin{table*}[htbp]
  \centering
  \caption{Base transformer architecture}
  \resizebox{0.75\textwidth}{!}{%
    \begin{tabular}{l|cccccc}
    \toprule
    \toprule
    \multicolumn{1}{p{4.785em}|}{\centering{\textbf{Hyper \newline{}Parameter}}} & \textbf{Layers} & \multicolumn{1}{p{3.43em}}{\centering{\textbf{Hidden \newline{}Size}}} & \multicolumn{1}{p{4.355em}}{\centering{\textbf{Attention\newline{} Heads}}} & \multicolumn{1}{p{7.5em}}{\centering{\textbf{Attention Heads\newline{} Size}}} & \multicolumn{1}{p{5.715em}}{\centering{\textbf{FFN\newline{} Hidden Size}}} & \multicolumn{1}{p{4.645em}}{\centering{\textbf{Sequence \newline{}Length}}} \\
    \midrule
    \textbf{Base} & 12    & 768   & 12    & 64    & 3072  & 384 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
  \label{tab:trans_arch}%
\end{table*}%

